Quantum influences and event relativity

We develop a new interpretation of quantum theory by combining insights from extended Wigner's friend scenarios and quantum causal modelling. In this interpretation, which synthesizes ideas from relational quantum mechanics and consistent histories, events obtain relative to a set of systems, and correspond to projectors that are picked out by causal structure. We articulate these ideas using a precise mathematical formalism. Using this formalism, we show through specific examples and general constructions how quantum phenomena can be modelled and paradoxes avoided; how different scenarios may be classified and the framework of quantum causal models extended; and how one can approach decoherence and emergent classicality without relying on quantum states.

==> bin.tex <==

\textbf{Bell} Consider the $(F, S)$ depicted in \ref{}. Suppose that $P_{Z}^i$, $P_{A}^a$, and $P_{B}^b$ do not form an irreducible interference fork. That is, suppose that each $P_{Z}^i$ can be written in the form $P_Z^i=\sum_{mn}Q_{Z}^{im}R_{Z}^{in}$, where $\{Q_{Z}^{im}\}$ and $\{R_{Z}^{in}\}$ are (commuting) projective decompositions on $\ch_{Z}$ (allowing that some $Q_{Z}^{im}$ and $R_{Z}^{in}$ may be the zero projector), and 
\begin{equation} \label{eq:no_int_1}
    \begin{split}
        \{Q_{Z}^{im}\} &\rightarrow \{P_B^b\} \\ 
        \{R_{Z}^{in}\} &\rightarrow \{P_A^a\} .
    \end{split}
\end{equation}

We can deduce two further absences of interference influences: (\ref{eq:fine_graining}) together with the fact that $X \not\rightarrow B$ and $Y \not\rightarrow A$ implies that 
\begin{equation} \label{eq:no_int_2}
\begin{split}
    \{P_X^x\} &\rightarrow \{P_B^b\} \\
    \{P_Y^y\} &\rightarrow \{P_A^a\}.
\end{split}
\end{equation}

Let us use tilde symbols to denote projectors that have been embedded into the Hilbert space for the whole circuit fragment and transformed into the ``time'' slice after $U$ but before $V$. So, for example, $\tilde{P}_A^a:=I_{W} \otimes \cv^\dag(P_A^a \otimes I_{FB})$, and $\tilde{Q_Z}^{im} := I_X \otimes \cu(Q_Z \otimes I_S) I_Y$. Now, consider the operator algebras
\begin{equation}
    \begin{split}
        \ca :&= \texttt{aspan}(\{\tilde{Q}_Z^{im}\} \cup \{\tilde{P}_X^x\} \cup \{\tilde{P}_A^a\}) \\
        \cb :&= \texttt{aspan}(\{\tilde{R}_Z^{in}\} \cup \{\tilde{P}_Y^y\} \cup \{\tilde{P}_B^b\}) 
    \end{split}
\end{equation}
where $\texttt{aspan}(s)$ is the algebra of operators obtained by taking matrix products and convex linear combinations of operators in the set $s$. Given the pseudo-temporal partial order induced by the cirucit, the only possible interferences influences between one of the three decompositons that generate $\ca$ and one of the three decompositions that generate $\cb$ are the ones already ruled out by (\ref{eq:no_int_1}) and (\ref{eq:no_int_2}). Recalling the the lack of an interference influence is equivalent to the commutation of the embedded Heisenberg projectors, it follows that $\ca \subseteq \texttt{comm}(\cb)$. Furthermore, any $M \in \ca$ can be written $M = M_{WXS} \otimes I_{Y}$ and any $N \in \cb$ can be written $I_{WX} \otimes M_{SY}$. It follows from Lemma \ref{lemma:structure} that there exists a decomposition $\ch_S = \bigoplus_k \ch_{S_L^k} \otimes \ch_{S_R^k}$ such elements of $\ca$ and $\cb$ can be written 
\begin{equation}
    \begin{split}
        \sum_k M_{WXS_L^k} \otimes \pi_{S_R^kY} \\
        \sum_k \pi_{WXS_L^k} \otimes N_{S_R^kY} 
    \end{split}
\end{equation}
respectively. 

We proceed to show that the indices $(m, n, k)$ define a hidden variable $\lambda$ with respect to which $p(axby|ij)$ admits a local hidden variable model for any fixed $i$ and $j$. A probability distribution over events corresponding to our original six decompositions is defined is follows:
\begin{equation}
    p(axbyij)= \frac{1}{d} {\rm Tr}(\tilde{P}_Z^i \tilde{P}_X^x \tilde{P}_Y^y\tilde{P}_W^j\tilde{P}_A^a\tilde{P}_B^b)    
\end{equation}
Mathematically, one can also write down a probability distribution
\begin{equation} \label{eq:eminem}
\begin{split}
       q(axbyijmnk)  := \frac{1}{d} {\rm Tr}(\tilde{Q_Z}^{im} \tilde{R_Z}^{in} \tilde{P}_S^k  \tilde{P}_X^x \tilde{P}_Y^y\tilde{P}_W^j\tilde{P}_A^a\tilde{P}_B^b)    
\end{split}
\end{equation}
where we have defined $\tilde{P}_S^k:=\pi_{WXS_L^k} \otimes \pi_{S_R^kY}$. (One way to verify that this is a valid probability distribution is start with the consistent histories formula (\ref{eqLch_prob}) and use a similar argument to the proof of Theorem \ref{thm:linear_prob} to show it reduces to the expression above.) And one can easily verify that $p(axbyij)=\sum_{mnk}q(axbyij\lambda)$, and hence that $p(axby|ij)=\sum_{mnk}q(axby\lambda|ij)$, where we have defined $\lambda:=mnk$. It remains to show that $q(axby|\lambda|ij)=(ax|\lambda|ij)(by|\lambda|ij)$ and $q(xy \lambda|ij)=q(xy|ij) q(\lambda|ij)$.

By commuting some operators around, we can rewrite $q(axbyijmnk)$ as
\begin{equation}
    \begin{split}
       q(axbyijmnk)  &= \frac{1}{d} {\rm Tr}(\tilde{P}_W^j \tilde{Q}_Z^{im}  \tilde{P}_X^x \tilde{P}_A^a \tilde{R}_Z^{in} \tilde{P}_Y^y \tilde{P}_B^b \tilde{P}_S^k)    \\
       &=\frac{1}{d} {\rm Tr}((P_W^j \otimes I_{XSY}) M^{imxa} N^{inyb} \tilde{P}_S^k)  \\
       &= \frac{1}{d} {\rm Tr}\big([(P_W^j \otimes \pi_{XS_L^k}) M^{imxa}_{WXS_L^k}] \otimes N^{inyb}_{S_R^kY} \big)  \\
       &=\frac{1}{d} {\rm Tr}([(P_W^j \otimes \pi_{XS_L^k}) M^{imxa}_{WXS_L^k}]) {\rm Tr}( N^{inyb}_{S_R^kY} )
    \end{split}
\end{equation}
More abstractly, we have shown that $q(axbyijmnk)$ can be written in terms of two functions $q(axbyijmnk) = f(axjimk)g(byink)$. Thus, adding in some trivial functional dependences, $q(axbyijmnk) = f(axjimnk)g(byimnk)$. Substituting $\lambda:=mnk$, this becomes
\begin{equation}
    q(axbyij\lambda) = f(axji \lambda)g(byi \lambda).
\end{equation}
Now, in general, if a probability distribution $p(\alpha \beta \gamma)=f(\alpha \gamma)g(\beta \gamma)$, it follows that $p(\alpha \beta \gamma)= p(\alpha|\gamma)p(\beta|\gamma)p(\gamma)$. Thus $q(axbyij\lambda)=q(axj|i\lambda)q(by|i\lambda)q(i \lambda)$. We now perform some manipulations: 
\begin{equation}
    \begin{split}
        q(axby|ij\lambda) &= \frac{q(axbyij\lambda)}{q(ij\lambda)} \\
        & = \frac{q(axj|i\lambda)q(by|i\lambda)}{q(j|i\lambda)  q(i\lambda)} \\
        &= \frac{q(ax|ij \lambda) q(by|i\lambda)}{ q(i\lambda)} \\
        &= q(ax|ij \lambda)q(by|ij \lambda)
    \end{split}
\end{equation}
And finally,
\begin{equation}
\begin{split}
        q(xy ij mnk ) &= \frac{1}{d} {\rm Tr}(\tilde{Q}_Z^{im}\tilde{R}_Z^{in}\tilde{P}_S^k \tilde{P}_W^j \tilde{P}_X^x \tilde{P}_Y^y ) \\ 
        &= \frac{1}{d} {\rm Tr}(O_{ZW}^{inmkj}) {\rm Tr}(P_X^x \otimes P_Y^y) \\
        &= f'(mnkij)g'(xy) \\
        &= f'(mnkij)g'(xyij) \\
        & \implies  q(xy ij \lambda)q(xy|ij) q(\lambda|ij)
\end{split}
\end{equation}
where the second line makes use of the fact that $\tilde{R}_Z^{i'n}\tilde{P}_S^k \tilde{P}_W^j$ has the form $O_{ZW}^{imnkj} \otimes I_{XY}$.




A consistent histories model of such an experiment might include the decomposition $\mathbb{D}_1=\{\ket{\psi}\bra{\psi}, I- \ket{\psi}\bra{\psi}\}$ for $t_1$ and $\mathbb{D}_3=\{\ket{\phi}\bra{\phi}, I- \ket{\phi}\bra{\phi}\}$ for $t_1$, together with the stipulation that the events corresponding to $\ket{\psi}\bra{\psi}$ and $\ket{\phi}\bra{\phi}$ happened at $t_1$ and $t_3$ respectively (throughout, we assume that time evolution is trivial). Such a model can be extended in one of two different ways. One could add in a decomposition $\mathbb{D}_2^i=\{\ket{i}\bra{i}, I - \ket{i}\bra{i}\}$ at time $t_2$ (where $t_3>t_2>t_1$) for either $i=0$ or $i=1$; in either case, the function (\ref{eqLch_prob}) for $\rho=I/d$ happens to be linear and the consistency condition is met. In the $i$th extension for each $i$, one finds from the probability function that the fact that the events for $\ket{\psi}\bra{\psi}$ and $\ket{\phi}\bra{\phi}$ both happened implies with certainty that an event corresponding to  $\ket{i}\bra{i}$ happens. In other words, relative to a choice of a consistent set of histories, the same initial data either implies the particle was definitely in the first box at $t_2$, or else that it was definitely in the second box.

This is not a logical contradiction, because the different inferences are made relative to different consistent sets. But, as Adrian Kent argues, it does undermine the motivating claim that consistent histories is the most minimal possible realist extension of the Copenhagen interpretation -- or even ``Copenhagen done right'' --, since there is no analogue of this phenomenon in the Copenhagen interpretation. And there does not appear to be any particular theoretical or experimental reason why one needs such models.

It is therefore encouraging that no such phenomenon takes place in our theory. Since $[\ket{\psi}\bra{\psi}, \ket{i}\bra{i}]\neq 0$ \textit{and} $[\ket{i}\bra{i}, \ket{\phi}\bra{\phi}] \neq 0$, (\ref{eq:allowed_int_infl}) implies that neither set of of three decompositions can all arise from the preference algorithm applied to a single bubble. Appendix \ref{app:3box} extends this argument to show that no three-box paradox can ever take place in our theory.
We note that similar remarks apply the quantum pigeonhole paradox \cite{aharonov2016quantum}, which can be formulated in a similar way using consistent histories.
When we take the stance that the physically significant consistent histories are the ones singled out by causal structure, we can recover the operational phenomena, explain the Wigner's friend scenario, and at the same time avoid unnecessary paradoxes.


ence algorithm, we can \textit{derive} linearity.

One is led to view e.g. $o_2$ as the outcome of measurement, because different choices of the second PVM will lead to different marginal probabilities $p(o_1, o_3, \ldots, o_N$), and these differences are explained by the idea that measurements disturb the system by inducing a nonlinear evolution, and different measurements disturb in different ways. But this explanation is based the problematically vague idea from standard quantum theory

it will help to recall the probability formula from the consistent histories formalism for $N$ events given some initial state $\rho$:
\begin{equation} \label{eqLch_prob}
    p(e_1, \ldots e_N) = {\rm Tr}(\tilde{P}_N^{e_N} \ldots \tilde{P}_1^{e_1}\rho \tilde{P}_1^{e_1} \ldots \tilde{P}_N^{e_N}),
\end{equation}
where the tildes denote that the projectors are being viewed as embedded in the overall Hilbert space, and in the Heisenberg picture (so we could rewrite the commutator from (\ref{eq:interference_influence_comm}) as $[\tilde{P}_A^i, \tilde{P}_D^j]$). 
Now, this function is not manifestly linear in each projector. In order to secure linearity\footnote{This is desirable since, without linearity, the probabilities obtained for a subset of $N-M$ events might be different depending on whether one calculates by marginalizing the above expression, or by directly applying a similar formula but missing out the projectors corresponding to the excluded events. For consistency, one would have to take the probabilities given by marginalization, but this is difficult to reconcile with the idea that all time evolution is unitary.}, the consistent histories formalism imposes a ``consistency'' condition by fiat, which ensures that this nonlinear function can be rewritten as a linear one (as explained in \cite{page1993no}). When decompositions are derived using the preference algorithm, however, there is no need to do this, due to the following theorem, to be proven shortly.



%%%%%%%%%%%%%%%%%%%%%%%%%%%


Sections \ref{sec:interpretation} and \ref{sec:consistent_histories} start with some useful background, first on the general problem of interpreting quantum theory, and then on the consistent histories formalism.
Section \ref{sec:influences} kicks off our own contributions by introducing the central notion of an \textit{interference influence}, which can be understood as the noncommutation of certain projectors in the Heisenberg picture. Section \ref{sec:events} shows how such influences lead to some sets of projectors being privileged by the causal structure of a unitary circuit -- at least relative to a given set of systems on the circuit, which we call a \textit{bubble}. These preferred sets of projectors give rise to a notion of (relational) events, which we can attribute probabilities with a simple linear trace rule.
Section \ref{sec:theory_models} turns these ideas into a precise theory with axioms; offers models of a prepare-measure experiment and the Wigner's friend scenario; and shows how the ``three-box paradox'' \cite{kent1997consistent} from consistent histories is avoided. 
It also points out that arbitrary circuits from operational quantum theory can be reproduced (proven in Appendix \ref{app:operational}), indicating that our theory finds itself in a ``Goldilocks zone'' with respect to the phenomena it can and cannot model.

Section \ref{sec:classications} uses the concept of an interference influence to classify five different types of quantum phenomena by the causal structures they require. This paves the way for an extension of the quantum causal modelling framework, and illuminates how our formalism and extensions thereof can provide an approach to decoherence based on a process ontology and not relying on quantum states.  Section \ref{sec:discussion} concludes with a discussion of where the formalism might be applied next, including the emergence of the classical world and quantum gravity. 




So does the preference algorithm single out consistent histories in which the sun rises? There are good reasons to think the answer is essentially ``yes'', at least relative to the right sort of bubbles. To take a somewhat comically simple toy model, if we take the \texttt{CNOT} defined earlier to describe the interaction between the sun and the earth, where $A/C$ is the sun and $B/D$ is the earth, $\mathbb{D}_A=\{\ket{0}\bra{0}_A, \ket{1}\bra{1}_A\}$ is the risen/not-risen degree of freedom of the sun at $t_1$ and  $\{\ket{0}\bra{0}_D, \ket{1}\bra{1}_D\}$ is a light/dark degree of freedom one face of the earth at a slightly later $t_2$, then we will indeed find that $\mathbb{D}_A$ of the sun is preferred relative to the bubble $\mathfrak{B}=\{A, D\}$. Note, however, one only gets the trivial decompositions $\{I_A\}$ and $\{I_C\}$ for the sun whenever both $A$ and $C$ is included. This is because the preference algorithm applied to such bubbles does not exclusively focus on the interaction between the sun and the earth; it also considers how the sun at $t_1$ influences itself at $t_2$.

More generally, since the interaction between systems tends to depend on their relative distance,  we expect systems that exert strong influences on other systems will become localized in bubbles that focus on the interaction.
Demonstrating this rigorously, and thus moving towards realistic accounts of the emergence of quasiclassical behavior, with a view to resolving the problems in \cite{dowker1996consistent}, is an important direction for future work. For now, however, we will set out our theory in detail in the case of finite-dimensional quantum theory.
